Approximate inference of marginals using the IBIA framework

Exact inference of marginals in probabilistic graphical models (PGM) is known to be intractable, necessitating the use of approximate methods. Most of the existing variational techniques perform iterative message passing in loopy graphs which is slow to converge for many benchmarks. In this paper, we propose a new algorithm for marginal inference that is based on the incremental build-infer-approximate (IBIA) paradigm. Our algorithm converts the PGM into a sequence of linked clique tree forests (SLCTF) with bounded clique sizes, and then uses a heuristic belief update algorithm to infer the marginals. For the special case of Bayesian networks, we show that if the incremental build step in IBIA uses the topological order of variables then (a) the prior marginals are consistent in all CTFs in the SLCTF and (b) the posterior marginals are consistent once all evidence variables are added to the SLCTF. In our approach, the belief propagation step is non-iterative and the accuracy-complexity trade-off is controlled using user-defined clique size bounds. Results for several benchmark sets from recent UAI competitions show that our method gives either better or comparable accuracy than existing variational and sampling based methods, with smaller runtimes.

==> findInterfaceLinks.tex <==
\subsection{Approximation: Create Interface Map (IM)}
In this step, we link cliques in $CTF_{in}$ and $CTF_a$.
For each clique $C'$ in $CTF_a$, we add a link to a clique or a set of cliques in $CTF_{in}$ in $IM$ as follows
\begin{itemize}
  \item If $C'$ is obtained after collapsing a set of cliques $\{C_1, \cdots C_m\}$ in $CTF_{in}$,  links are added from $C'$ to each of $\{C_1, \cdots C_m\}$.
    \item If $C'$ is obtained from $C$ in $CTF_{in}$ after a local marginalization, a link is added from $C'$ to $C$.
  \item If $C'$ is same as clique $C$ in $CTF_{in}$, a link is added from $C'$ to $C$.
\end{itemize}
$IM$ is implemented as a Python dictionary, with cliques $C'$ in $CTF_a$ used as keys and the corresponding cliques in $CTF_{in}$ as values i.e. $IM[C']=\{C\}$.

\subsection{Updating links between adjacent CTFs}\label{sec:links}
The build, infer and approximate steps are used repeatedly until all variables are added to some CTF in the SLCTF. At this point, we have a sequence of CTFs and interface maps between each CTF and its approximation.
In this section, we discuss the method to update the interface map $IM$ so that it contains links between adjacent CTFs. As will be seen in Section~\ref{sec:pm}, these links are needed for computation of the posterior marginals, $MAR_e$.
%to update beliefs in order to account for all evidence variables.

\input{tikz/links}
We first show the process using the running example. As shown in Figure~\ref{fig:approxCTF1}, we have added links between cliques in $CTF_1$ and $CTF_{1,a}$ to $IM_1$. 
Figure~\ref{fig:links} shows the two CTFs, $CTF_1$ and $CTF_2$ in the SLCTF obtained for the running example as well as the updated $IM_1$. 
$CTF_2$ is incrementally built by adding the variables $p$ and $q$ to $CTF_{1,a}$. Therefore, each clique $C'$ in $CTF_{1,a}$ will be contained in some clique $\tilde{C}$ in $CTF_2$. As shown in Figure~\ref{fig:links}, we add a link between $C'$ and $\tilde{C}$ in $IM_1$. For example, the variables in both ${C_1}'$ and ${C_2}'$ are contained in $\tilde{C_2}$. Hence, both cliques are linked to $\tilde{C_2}$. 

%We update the interface map by adding cliques in $CTF_2$ that contain the corresponding cliques in $CTF_{1,a}$. Figure~\ref{fig:links} shows the updated interface map and  the final set of links.

Algorithm \ref{alg:updateInterfaceMap} describes the procedure used to update the links. 
%The links are updated as follows.
$CTF_{k}$ and $CTF_{k,a}$ denote the $k^{th}$ CTF in the sequence and its approximation respectively. $CTF_{k+1}$ is the next CTF in the sequence. 
%While building $CTF_{k+1}$, a clique $C_j'$ in $CTF_{k,a}$ could morph into new clique $\tilde{C}_j$.
%We update the interface map by adding a clique $\tilde{C_j}$ in $CTF_{k+1}$ for each  ${C_j}'$ in the dictionary $IM_{k}$ such that ${C_j}'$ is a subset of $\tilde{C_j}$. 
%The approximate $CTF_{k,a}$ forms the starting point for $CTF_{k+1}$. 
%The variables in $CTF_{k,a}$ are denoted {\textbf{link variables}}. These variables are present in both $CTF_{k}$ and $CTF_{k+1}$.
$IM_k$ is the interface map that contains links between cliques in $CTF_k$ and $CTF_{k,a}$. 
Since $CTF_{k+1}$ is constructed by incrementally adding variables to $CTF_{k,a}$,  each clique ${C_j}'$ in $CTF_{k,a}$ is contained in some clique $\tilde{C_j}$ in $CTF_{k+1}$. 
We update the interface map by adding a clique $\tilde{C_j}$ for each  ${C_j}'$ in the dictionary $IM_{k}$ such that ${C_j}'$ is a subset of $\tilde{C_j}$. 
At the end of this step, each  ${C_j}'$ in $IM_{k}$ has links to one or more cliques in the $CTF_{k}$ and a link to a clique in $CTF_{k+1}$.
The variables in $CTF_{k,a}$ are called the link variables (Definition~\ref{def:lv}, section~\ref{sec:definitions}). The link variables associated with the link between between cliques $C_j\in CTF_k$ and $\tilde{C_j}\in CTF_{k+1}$ is the set $L=C_j\cap {C_j}'$.
%Corresponding to the link between cliques $C_j\in CTF_k$ and $\tilde{C_j}\in CTF_{k+1}$, we denote the variables in the set $C_j\cap {C_j}'$ as \textbf{link variables}.
\input{Algo_updateLinks}




==> tables/averageHD1.tex <==
\begin{table}[!htp]\centering
    \caption{Comparison of average $HD_{avg}$ and average $HD_{max}$ (shown in gray background) obtained using various inference methods with two runtime constraints, 2 min and 20 min. The minimum error obtained for each time limit is highlighted in bold. Entries are marked as ‘-’ where all instances could not be solved within the set time limit. The total number of instances solved by each method is shown in the last row. $v_a$: average number of variables, $f_a$: average number of factors, $w_a$: average induced width and $dm_a$: average of the maximum variable domain size.
    }
\label{tab:smallInst}
\small
    \setlength\tabcolsep{3pt}
    \begin{tabular}{llllllllllll}\toprule
        \multirow{2}{*}{} &Total &\multirow{2}{*}{$(v_a,f_a,w_a,dm_a)$} &\multicolumn{4}{c}{2 min} &\multicolumn{4}{c}{20 min} \\\cmidrule(lr){4-7}\cmidrule(lr){8-11}
&\#Inst & &LBP &IJGP &ISSwc &IBIA20 &LBP &IJGP &ISSwc &IBIA23 \\\midrule
BN &97 &(637,637,28,10) &- &- &- &\textbf{2E-4} &0.023 &- &- &\textbf{6E-5} \\
\rowcolor{gray!20}& & &- &- &- &\textbf{9E-3} &0.230 &- &- &\textbf{2E-3} \\
GridBN &29 &(595,595,37,2) &0.075 &0.011 &0.003 &\textbf{5E-6} &0.075 &0.010 &0.001 &\textbf{2E-7} \\
\rowcolor{gray!20}& & &0.478 &0.111 &0.051 &\textbf{7E-4} &0.478 &0.094 &0.015 &\textbf{1E-4} \\
Bnlearn &26 &(256,256,7,16) &0.010 &0.011 &0.012 &\textbf{7E-5} &0.010 &0.008 &0.006 &\textbf{7E-6} \\
\rowcolor{gray!20}& & &0.089 &0.050 &0.064 &\textbf{0.002} &0.089 &0.025 &0.028 &\textbf{2E-4} \\
Pedigree &24 &(853,853,24,5) &0.075 &0.035 &0.033 &\textbf{0.009} &0.075 &0.033 &0.021 &\textbf{0.008} \\
\rowcolor{gray!20}& & &0.555 &0.470 &0.292 &\textbf{0.204} &0.555 &0.446 &0.234 &\textbf{0.198} \\
Promedas &64 &(618,618,21,2) &0.032 &0.124 &0.030 &\textbf{0.013} &0.032 &0.120 &0.021 &\textbf{0.010} \\
\rowcolor{gray!20}& & &0.168 &0.504 &0.139 &\textbf{0.086} &0.168 &0.487 &0.096 &\textbf{0.072} \\
DBN &36 &(719,14205,29,2) &- &0.081 &\textbf{0.016} &0.020 &- &0.060 &\textbf{2E-6} &0.003 \\
\rowcolor{gray!20}& & &- &0.919 &0.766 &\textbf{0.261} &- &0.879 &\textbf{2E-4} &0.098 \\
ObjDetect &79 &(60,210,6,16) &0.022 &0.004 &0.018 &\textbf{0.002} &0.022 &\textbf{3E-5} &0.009 &4E-4 \\
\rowcolor{gray!20}& & &0.130 &0.037 &0.189 &\textbf{0.020} &0.130 &\textbf{3E-4} &0.061 &0.006 \\
Grids &8 &(250,728,22,2) &0.433 &0.247 &- &\textbf{0.088} &0.433 &0.123 &0.056 &\textbf{0.002} \\
\rowcolor{gray!20}& & &0.905 &0.713 &- &\textbf{0.300} &0.905 &0.423 &0.209 &\textbf{0.099} \\
CSP &12 &(73,369,12,4) &0.019 &0.026 &- &\textbf{0.002} &0.019 &0.017 &0.054 &\textbf{2E-4} \\
\rowcolor{gray!20}& & &0.066 &0.134 &- &\textbf{0.011} &0.066 &0.073 &0.093 &\textbf{0.003} \\
Segment &50 &(229,851,17,2) &0.035 &\textbf{5E-6} &\textbf{5E-6} &6E-5 &0.035 &5E-6 &5E-6 &\textbf{1E-7} \\
\rowcolor{gray!20}& & &0.258 &\textbf{7E-5} &\textbf{7E-5} &0.001 &0.258 &7E-5 &7E-5 &\textbf{4E-7} \\
Protein &68 &(59,176,6,77) &\textbf{5E-4} &0.003 &0.003 &6E-4 &5E-4 &0.007 &0.001 &\textbf{3E-5} \\
\rowcolor{gray!20}& & &\textbf{0.007} &0.094 &0.049 &0.039 &0.007 &0.230 &0.015 &\textbf{0.002} \\ 
\midrule
\#Inst &493 & &481 &487 &485 &493 &485 &491 &487 &493 \\
\bottomrule
\end{tabular}
\end{table}




%\begin{table}[!htp]\centering
%\caption{Comparison of error in marginals obtained with various inference methods measured using two error metrics. We compare results obtained with two runtime constraints, 2 minutes and 20 minutes. The minimum error obtained for each set in highlighted in bold. Entries are marked as ‘-’ where all instances could not solved within the set time limit. The total number instances solved by each method is highlighted in gray. $v_a$: average number of variables, $f_a$: average number of factors, $w_a$: average induced width and $dm_a$: average of the maximum variable domain size.
%    }
%\label{tab:smallInst}
%\begin{subtable}{\textwidth}
%\centering
%    \caption{Average of $HD_{avg}$ over all instances in each benchmark set.}\label{tab:avgHD}
%\label{tab:}
%\scriptsize
%\setlength\tabcolsep{3pt}
%\begin{tabular}{lrrrrrrrrrrrr}\toprule
%\multirow{2}{*}{} &Total &\multirow{2}{*}{$(v_a,f_a,w_a,dm_a)$} &\multicolumn{5}{c}{2 minutes} &\multicolumn{4}{c}{20 minutes} \\ \cmidrule(lr){4-8}\cmidrule(lr){9-12}
%&\#Inst & &LBP &HAK &ISSwc20 &ISSwcd &IBIA20 &ISSwc20 &ISSwcd &IBIA20 &IBIA23 \\\midrule
%BN &97 &(637,637,28,10) &- &- &0.037 &- &\textbf{2E-4} &0.033 &- &2E-4 &\textbf{6E-5} \\
%GridBN &29 &(595,595,37,2) &0.075 &0.018 &0.005 &0.003 &\textbf{5E-6} &0.005 &0.001 &5E-6 &\textbf{2E-7} \\
%Bnlearn &26 &(256,256,7,16) &0.010 &0.021 &0.036 &0.012 &\textbf{7E-5} &0.036 &0.006 &7E-5 &\textbf{7E-6} \\
%Pedigree &24 &(853,853,24,5) &0.075 &0.034 &0.028 &0.033 &\textbf{0.009} &0.021 &0.021 &0.009 &\textbf{0.008} \\
%Promedas &64 &(618,618,21,2) &0.032 &0.033 &0.042 &0.030 &\textbf{0.013} &0.033 &0.021 &0.013 &\textbf{0.010} \\
%DBN &36 &(719,14205,29,2) &- &0.284 &\textbf{0.011} &0.016 &0.020 &\textbf{2E-6} &\textbf{2E-6} &0.020 &0.003 \\
%ObjDetect&79 &(60,210,6,16) &0.022 &0.085 &0.039 &0.018 &\textbf{0.002} &0.004 &0.009 &0.002 &\textbf{4E-4} \\
%Grids &8 &(250,728,22,2) &0.433 &0.323 &- &- &0.088 &- &0.056 &0.088 &\textbf{0.002} \\
%CSP &12 &(73,369,12,4) &0.019 &0.038 &- &- &\textbf{0.002} &0.069 &0.054 &0.002 &\textbf{2E-4} \\
%Segment &50 &(229,851,17,2) &0.035 &0.007 &0.002 &\textbf{5E-6} &6E-5 &5E-6 &5E-6 &6E-5 &\textbf{1E-7} \\
%Protein &68 &(59,176,6,77) &- &- &0.003 &0.003 &\textbf{6E-4} &0.001 &0.001 &6E-4 &\textbf{3E-5} \\
%    \midrule
%    \rowcolor{gray!20}\#Inst.&493 & & \cellcolor{red!20}& \cellcolor{red!20} &488 &485 &493 &489 &487 &493 &493  \\
% %   \rowcolor{gray!20}solved && & & & & & & & & & &  \\
%\bottomrule
%\end{tabular}
%\end{subtable}
%
%\begin{subtable}{\textwidth}
%\centering
%    \caption{Average of $AE_{max}$ over all instances in each benchmark set}\label{tab:maxError}
%    %\small
%    \scriptsize
%\setlength\tabcolsep{3pt}
%\begin{tabular}{lrrrrrrrrrrrr}\toprule
%    &Total &\multirow{2}{*}{$(v_a,f_a,w_a,dm_a)$} &\multicolumn{5}{c}{2 minutes} &\multicolumn{4}{c}{20 minutes} \\\cmidrule(lr){4-8}\cmidrule(lr){9-12}
%&\#Inst & &LBP &HAK &ISSwc20 &ISSwcd &IBIA20 &ISSwc20 &ISSwcd &IBIA20 &IBIA23 \\\midrule
%BN &97 &(637,637,28,10) &- &- &0.151 &- &\textbf{0.005} &0.090 &- &0.005 &\textbf{0.001} \\
%GridBN &29 &(595,595,37,2) &0.474 &0.206 &0.073 &0.059 &\textbf{9E-4} &0.053 &0.020 &9E-4 &\textbf{1E-4} \\
%Bnlearn &26 &(256,256,7,16) &0.068 &0.092 &0.093 &0.051 &\textbf{7E-4} &0.092 &0.024 &7E-4 &\textbf{1E-4} \\
%Pedigree &24 &(853,853,24,5) &0.534 &0.405 &\textbf{0.254} &0.316 &0.263 &\textbf{0.211} &0.248 &0.263 &0.242 \\
%Promedas &64 &(618,618,21,2) &0.166 &0.163 &0.220 &0.148 &\textbf{0.080} &0.163 &0.102 &0.080 &\textbf{0.064} \\
%DBN &36 &(719,14205,29,2) &- &0.477 &0.833 &0.761 &\textbf{0.287} &\textbf{5E-7} &\textbf{5E-7} &0.287 &0.100 \\
%ObjDetect &79 &(60,210,6,16) &0.081 &0.289 &0.195 &0.109 &\textbf{0.009} &0.009 &0.042 &0.009 &\textbf{0.003} \\
%Grids &8 &(250,728,22,2) &0.940 &0.480 &- &- &\textbf{0.339} &- &0.224 &0.339 &\textbf{0.109} \\
%CSP &12 &(73,369,12,4) &0.061 &0.128 &- &- &\textbf{0.006} &0.083 &0.104 &0.006 &\textbf{0.002} \\
%Segment &50 &(229,851,17,2) &0.243 &0.042 &0.037 &\textbf{5E-7} &8E-4 &7E-7 &\textbf{5E-7} &8E-4 &\textbf{5E-7} \\
%Protein &68 &(59,176,6,77) &- &- &\textbf{0.017} &0.025 &0.040 &0.005 &0.008 &0.040 &\textbf{8E-4} \\
%\bottomrule
%\end{tabular}
%\end{subtable}
%\end{table}



==> tables/cutset.tex <==
\begin{table}[!htp]\centering
\caption{Comparison of error obtained with sample search with and without cutset sampling (CS). The runtime limit was set to 2 minutes and ibound was set to default value determined by the solver.}\label{tab: }
\small
\begin{tabular}{lrrrrrr}\toprule
\multirow{2}{*}{} &\multirow{2}{*}{\#Inst} &\multicolumn{2}{c}{Avg. $HD_{mean}$} &\multicolumn{2}{c}{Avg. $MaxAbsErr$} \\\cmidrule{3-6}
& &with CS &without CS &with CS &without CS \\\midrule
BN &97 &- &- &- &- \\
GridBN &29 &0.003 &0.136 &0.059 &0.523 \\
Bnlearn &26 &0.012 &- &0.051 &- \\
Pedigree &24 &0.033 &0.243 &0.316 &0.772 \\
Promedas &64 &0.030 &0.146 &0.148 &0.683 \\
DBN &36 &0.016 &0.055 &0.761 &0.125 \\
Object Detection &79 &0.018 &0.019 &0.109 &0.030 \\
Grids &8 &- &0.411 &- &0.972 \\
CSP &12 &- &0.062 &- &0.110 \\
Segmentation &50 &5E-6 &0.013 &5E-7 &0.055 \\
Protein &68 &0.003 &9E-4 &0.025 &0.002 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/data.tex <==
\begin{table}[!htp]\centering
\caption{Generated by Spread-LaTeX}\label{tab: }
\scriptsize
\begin{tabular}{lrrrrrrrrr}\toprule
    & & & \multicolumn{6}{c}{Average $HD_{avg}$ / Average $HD_{max}$}\\ \cmidrule{4-9}
\multirow{2}{*}{} &Total &\multirow{2}{*}{$(v_a,f_a,w_a,dm_a)$} &\multicolumn{6}{c}{2 minutes} \\\cmidrule{2-2}\cmidrule{4-9}
&\#Inst & &LBP &HAK &IJGP &ISSwcd &ISSwc20 &IBIA20 \\\midrule
BN &97 &(637,637,28,10) &- &- &- &- &0.037 &\textbf{2E-4} \\
& & &- &- &- &- &0.145 &\textbf{9E-3} \\
GridBN &29 &(595,595,37,2) &0.075 &0.018 &0.011 &0.003 &0.005 &\textbf{5E-6} \\
& & &0.478 &0.234 &0.111 &0.051 &0.065 &\textbf{7E-4} \\
Bnlearn &26 &(256,256,7,16) &0.010 &0.021 &0.011 &0.012 &0.036 &\textbf{7E-5} \\
& & &0.089 &0.103 &0.050 &0.064 &0.094 &\textbf{0.002} \\
Pedigree &24 &(853,853,24,5) &0.075 &0.034 &0.035 &0.033 &0.028 &\textbf{0.009} \\
& & &0.555 &0.364 &0.470 &0.292 &0.245 &\textbf{0.204} \\
Promedas &64 &(618,618,21,2) &0.032 &0.033 &0.124 &0.030 &0.042 &\textbf{0.013} \\
& & &0.168 &0.158 &0.504 &0.139 &0.207 &\textbf{0.086} \\
DBN &36 &(719,14205,29,2) &- &0.284 &0.081 &0.016 &\textbf{0.011} &0.020 \\
& & &- &0.502 &0.919 &0.766 &0.833 &\textbf{0.261} \\
ObjDetect &79 &(60,210,6,16) &0.022 &0.085 &0.004 &0.018 &0.039 &\textbf{0.002} \\
& & &0.130 &0.325 &0.037 &0.189 &0.233 &\textbf{0.020} \\
Grids &8 &(250,728,22,2) &0.433 &0.323 &0.247 &- &- &\textbf{0.088} \\
& & &0.905 &0.495 &0.713 &- &- &\textbf{0.300} \\
CSP &12 &(73,369,12,4) &0.019 &0.038 &0.026 &- &- &\textbf{0.002} \\
& & &0.066 &0.118 &0.134 &- &- &\textbf{0.011} \\
Segment &50 &(229,851,17,2) &0.035 &0.007 &\textbf{5E-6} &\textbf{5E-6} &0.002 &6E-5 \\
& & &0.258 &0.058 &\textbf{7E-5} &\textbf{7E-5} &0.036 &0.001 \\
Protein &68 &(59,176,6,77) &\textbf{5E-4} &- &0.003 &0.003 &0.003 &\textbf{6E-4} \\
& & &\textbf{0.007} &- &0.094 &0.049 &0.030 &0.039 \\ \midrule
\rowcolor{gray!20}\#Inst &493 & &481 &458 &487 &485 &488 &493 \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[!htp]\centering
\caption{Generated by Spread-LaTeX}\label{tab: }
\scriptsize
\begin{tabular}{lrrrrrrrrrr}\toprule
    & & & \multicolumn{7}{c}{Average $HD_{avg}$ / Average $HD_{max}$}\\ \cmidrule{4-10}
\multirow{2}{*}{} &Total &\multirow{2}{*}{$(v_a,f_a,w_a,dm_a)$} &\multicolumn{7}{c}{20 minutes} \\\cmidrule{2-2}\cmidrule{4-10}
&\#Inst & &LBP &HAK &IJGP &ISSwcd &ISSwc20 &IBIA20 &IBIA23 \\\midrule
BN &97 &(637,637,28,10) &0.023 &- &- &- &0.033 &2E-4 &\textbf{6E-5} \\
& & &0.230 &- &- &- &0.085 &9E-3 &\textbf{2E-3} \\
GridBN &29 &(595,595,37,2) &0.075 &- &0.010 &0.001 &0.005 &5E-6 &\textbf{2E-7} \\
& & &0.478 &- &0.094 &0.015 &0.046 &7E-4 &\textbf{1E-4} \\
Bnlearn &26 &(256,256,7,16) &0.010 &0.010 &0.008 &0.006 &0.036 &7E-5 &\textbf{7E-6} \\
& & &0.089 &0.075 &0.025 &0.028 &0.093 &2E-3 &\textbf{2E-4} \\
Pedigree &24 &(853,853,24,5) &0.075 &0.036 &0.033 &0.021 &0.021 &0.009 &\textbf{0.008} \\
& & &0.555 &0.388 &0.446 &0.234 &\textbf{0.195} &0.204 &0.198 \\
Promedas &64 &(618,618,21,2) &0.032 &0.032 &0.120 &0.021 &0.033 &0.013 &\textbf{0.010} \\
& & &0.168 &0.168 &0.487 &0.096 &0.153 &0.086 &\textbf{0.072} \\
DBN &36 &(719,14205,29,2) &- &0.284 &0.060 &\textbf{2E-6} &\textbf{2E-6} &0.020 &0.003 \\
& & &- &0.501 &0.879 &\textbf{2E-4} &\textbf{2E-4} &0.261 &0.098 \\
ObjDetect &79 &(60,210,6,16) &0.022 &- &\textbf{3E-5} &0.009 &0.004 &0.002 &4E-4 \\
& & &0.130 &- &\textbf{3E-4} &0.061 &0.021 &0.020 &0.006 \\
Grids &8 &(250,728,22,2) &0.433 &0.324 &0.123 &0.056 &- &0.088 &\textbf{0.002} \\
& & &0.905 &0.496 &0.423 &0.209 &- &0.300 &\textbf{0.099} \\
CSP &12 &(73,369,12,4) &0.019 &0.031 &0.017 &0.054 &0.069 &0.002 &\textbf{2E-4} \\
& & &0.066 &0.084 &0.073 &0.093 &0.081 &0.011 &\textbf{0.003} \\
Segment &50 &(229,851,17,2) &0.035 &0.005 &5E-6 &5E-6 &5E-6 &6E-5 &\textbf{1E-7} \\
& & &0.258 &0.039 &7E-5 &7E-5 &7E-5 &0.001 &\textbf{4E-7} \\
Protein &68 &(59,176,6,77) &\textbf{5E-4} &- &0.007 &0.001 &0.001 &6E-4 &\textbf{3E-5} \\
& & &\textbf{0.007} &- &0.230 &0.015 &0.011 &0.039 &\textbf{0.002} \\ \midrule
\rowcolor{gray!20} \#Inst &493 & &485 &449 &491 &487 &489 &493 &493 \\
\bottomrule
\end{tabular}
\end{table}



==> tables/ijgp.tex <==
\begin{table}[!htp]\centering
\caption{Comparison of error in marginals estimated using IJGP, ISSwcd, ISSwc20 and IBIA20. Parameter $ibound$ sets the maximum number of variables in a cluster for IJGP and the maximum effective number of binary variables in ISSwcd, ISSwc20 and IBIA20. IJGP starts with the minimum value for $ibound$ and increases it until the runtime and memory constraints are satisfied.}\label{tab: }
\scriptsize
\begin{tabular}{lrrrrr|rrrrr}\toprule
& &\multicolumn{4}{c|}{$HD_{avg}$} &\multicolumn{4}{c}{$AE_{max}$} \\\cmidrule{3-10}
&\#Inst &IJGP &ISSwc20 &ISSwcd &IBIA20 &IJGP &ISSwc20 &ISSwcd &IBIA20 \\\midrule
BN &97 &- &0.037 &- &\textbf{2E-4} &- &0.151 &- &\textbf{0.005} \\
GridBN &29 &0.011 &0.005 &0.003 &\textbf{5E-6} &0.121 &0.073 &0.059 &\textbf{9E-4} \\
Bnlearn &26 &0.011 &0.036 &0.012 &\textbf{7E-5} &0.058 &0.093 &0.051 &\textbf{7E-4} \\
Pedigree &24 &0.035 &0.028 &0.033 &\textbf{0.009} &0.554 &\textbf{0.254} &0.316 &0.263 \\
Promedas &64 &0.124 &0.042 &0.030 &\textbf{0.013} &0.569 &0.220 &0.148 &\textbf{0.080} \\
DBN &36 &0.081 &\textbf{0.011} &0.016 &0.020 &0.920 &0.833 &0.761 &\textbf{0.287} \\
Object Detection &79 &0.004 &0.039 &0.018 &\textbf{0.002} &0.017 &0.195 &0.109 &\textbf{0.009} \\
Grids &8 &0.247 &- &- &0.088 &0.774 &- &- &\textbf{0.339} \\
CSP &12 &0.026 &- &- &\textbf{0.002} &0.154 &- &- &\textbf{0.006} \\
Segmentation &50 &5E-6 &0.002 &5E-6 &6E-5 &\textbf{5E-7} &0.037 &\textbf{5E-7} &8E-4 \\
Protein &68 &0.003 &0.003 &0.003 &\textbf{6E-4} &0.094 &\textbf{0.017} &0.025 &0.040 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/ijgpss.tex <==
\begin{table}[!htp]\centering
    \caption{Comparison of average $HD_{avg}$ and average $HD_{max}$ (shown in gray background) obtained using IBIA with $mcs_p=20$ (IBIA20), ISSwc with clique size bounds determined by the solver~\citep{ijgpss} (ISSwcd) and ISSwc with $ibound$ and $w\mbox{-}cutset$ bound fixed to 20 (ISSwc20). Results are shown for two runtime limits, 2 min and 20 min.  Entries are marked with `-' if the solution for all testcases could not be obtained within the given time and memory limits. The minimum error obtained for a benchmark is highlighted in bold.
    The number of instances solved by each solver is shown in the last row.
    $v_a$: average number of variables, $f_a$: average number of factors, $w_a$: average induced width and $dm_a$: average of the maximum variable domain size.
    }\label{tab:ijgpss}
\small
\begin{tabular}{lrrrrrrrr}\toprule
    \multirow{2}{*}{} &Total &\multirow{2}{*}{$(v_a,f_a,w_a,dm_a)$} &\multicolumn{3}{c}{2 min} &\multicolumn{2}{c}{20 min} \\\cmidrule(lr){4-6}\cmidrule(lr){7-8}
&\#Inst & &ISSwcd &ISSwc20 &IBIA20 &ISSwcd &ISSwc20 \\\midrule
BN &97 &(637,637,28,10) &- &0.037 &\textbf{2E-4} &- &0.033 \\
\rowcolor{gray!20}& & &- &0.145 &\textbf{9E-3} &- &0.085 \\
GridBN &29 &(595,595,37,2) &0.003 &0.005 &\textbf{5E-6} &0.001 &0.005 \\
\rowcolor{gray!20}& & &0.051 &0.065 &\textbf{7E-4} &0.015 &0.046 \\
Bnlearn &26 &(256,256,7,16) &0.012 &0.036 &\textbf{7E-5} &0.006 &0.036 \\
\rowcolor{gray!20}& & &0.064 &0.094 &\textbf{0.002} &0.028 &0.093 \\
Pedigree &24 &(853,853,24,5) &0.033 &0.028 &\textbf{0.009} &0.021 &0.021 \\
    \rowcolor{gray!20}& & &0.292 &0.245 &0.204 &0.234 &\textbf{0.195} \\
Promedas &64 &(618,618,21,2) &0.030 &0.042 &\textbf{0.013} &0.021 &0.033 \\
\rowcolor{gray!20}& & &0.139 &0.207 &\textbf{0.086} &0.096 &0.153 \\
DBN &36 &(719,14205,29,2) &0.016 &0.011 &0.020 &\textbf{2E-6} &\textbf{2E-6} \\
\rowcolor{gray!20}& & &0.766 &0.833 &0.261 &\textbf{2E-4} &\textbf{2E-4} \\
ObjDetect &79 &(60,210,6,16) &0.018 &0.039 &\textbf{0.002} &0.009 &0.004 \\
\rowcolor{gray!20}& & &0.189 &0.233 &\textbf{0.020} &0.061 &0.021 \\
    Grids &8 &(250,728,22,2) &- &- &0.088 &\textbf{0.056} &- \\
    \rowcolor{gray!20}& & &- &- &0.300 &\textbf{0.209} &- \\
CSP &12 &(73,369,12,4) &- &- &\textbf{0.002} &0.054 &0.069 \\
\rowcolor{gray!20}& & &- &- &\textbf{0.011} &0.093 &0.081 \\
Segment &50 &(229,851,17,2) &\textbf{5E-6} &0.002 &6E-5 &\textbf{5E-6} &\textbf{5E-6} \\
\rowcolor{gray!20}& & &\textbf{7E-5} &0.036 &0.001 &\textbf{7E-5} &\textbf{7E-5} \\
Protein &68 &(59,176,6,77) &0.003 &0.003 &\textbf{6E-4} &0.001 &0.001 \\
\rowcolor{gray!20}& & &0.049 &0.030 &0.039 &0.015 &\textbf{0.011} \\
\midrule
\#Inst &493 & &485 &488 &493 &487 &489 \\
\bottomrule
\end{tabular}
%\begin{tabular}{lrrrrrrrrr}\toprule
%    \multirow{2}{*}{} &Total &\multirow{2}{*}{$(v_a,f_a,w_a,dm_a)$} &\multicolumn{3}{c}{2 min} &\multicolumn{3}{c}{20 min} \\\cmidrule(lr){4-6}\cmidrule{7-9}
%&\#Inst & &ISSwc &ISSwc20 &IBIA20 &ISSwc &ISSwc20 &IBIA23 \\\midrule
%BN &97 &(637,637,28,10) &- &0.037 &\textbf{2E-4} &- &0.033 &\textbf{6E-5} \\
%\rowcolor{gray!20}& & &- &0.145 &\textbf{9E-3} &- &0.085 &\textbf{2E-3} \\
%GridBN &29 &(595,595,37,2) &0.003 &0.005 &\textbf{5E-6} &0.001 &0.005 &\textbf{2E-7} \\
%\rowcolor{gray!20}& & &0.051 &0.065 &\textbf{7E-4} &0.015 &0.046 &\textbf{1E-4} \\
%Bnlearn &26 &(256,256,7,16) &0.012 &0.036 &\textbf{7E-5} &0.006 &0.036 &\textbf{7E-6} \\
%\rowcolor{gray!20}& & &0.064 &0.094 &\textbf{0.002} &0.028 &0.093 &\textbf{2E-4} \\
%Pedigree &24 &(853,853,24,5) &0.033 &0.028 &\textbf{0.009} &0.021 &0.021 &\textbf{0.008} \\
%\rowcolor{gray!20}& & &0.292 &0.245 &\textbf{0.204} &0.234 &0.195 &\textbf{0.198} \\
%Promedas &64 &(618,618,21,2) &0.030 &0.042 &\textbf{0.013} &0.021 &0.033 &\textbf{0.010} \\
%\rowcolor{gray!20}& & &0.139 &0.207 &\textbf{0.086} &0.096 &0.153 &\textbf{0.072} \\
%DBN &36 &(719,14205,29,2) &0.016 &\textbf{0.011} &0.020 &\textbf{2E-6} &\textbf{2E-6} &0.003 \\
%\rowcolor{gray!20}& & &0.766 &0.833 &\textbf{0.261} &\textbf{2E-4} &\textbf{2E-4} &0.098 \\
%ObjDetect &79 &(60,210,6,16) &0.018 &0.039 &\textbf{0.002} &0.009 &0.004 &\textbf{4E-4} \\
%\rowcolor{gray!20}& & &0.189 &0.233 &\textbf{0.020} &0.061 &0.021 &\textbf{0.006} \\
%Grids &8 &(250,728,22,2) &- &- &\textbf{0.088} &0.056 &- &\textbf{0.002} \\
%\rowcolor{gray!20}& & &- &- &\textbf{0.300} &0.209 &- &\textbf{0.099} \\
%CSP &12 &(73,369,12,4) &- &- &\textbf{0.002} &0.054 &0.069 &\textbf{2E-4} \\
%\rowcolor{gray!20}& & &- &- &\textbf{0.011} &0.093 &0.081 &\textbf{0.003} \\
%Segment &50 &(229,851,17,2) &\textbf{5E-6} &0.002 &6E-5 &5E-6 &5E-6 &\textbf{1E-7} \\
%\rowcolor{gray!20}& & &\textbf{7E-5} &0.036 &0.001 &7E-5 &7E-5 &\textbf{4E-7} \\
%Protein &68 &(59,176,6,77) &0.003 &0.003 &\textbf{6E-4} &0.001 &0.001 &\textbf{3E-5} \\
%\rowcolor{gray!20}& & &0.049 &\textbf{0.030} &0.039 &0.015 &0.011 &\textbf{0.002} \\
%\midrule
%\#Inst &493 & &485 &488 &493 &487 &489 &493 \\
%\bottomrule
%\end{tabular}
%\begin{tabular}{lrrrrrrr}\toprule
% %   & & & \multicolumn{4}{c}{Average $HD_{avg}$ / Average $HD_{max}$}\\ \cmidrule{4-7}
%\multirow{2}{*}{} &Total &\multirow{2}{*}{$(v_a,f_a,w_a,dm_a)$} &\multicolumn{2}{c}{2 min} &\multicolumn{2}{c}{20 min} \\\cmidrule(lr){4-5}\cmidrule(lr){6-7}
%&\#Inst & &ISSwcd &ISSwc20 &ISSwcd &ISSwc20 \\\midrule
%BN &97 &(637,637,28,10) &- &0.037&- &0.033\\
%\rowcolor{gray!20}& & &- &0.145&- &0.085\\
%GridBN &29 &(595,595,37,2) &0.003&0.005 &0.001&0.005 \\
%\rowcolor{gray!20}& & &0.051&0.065 &0.015&0.046 \\
%Bnlearn &26 &(256,256,7,16) &0.012&0.036 &0.006&0.036 \\
%\rowcolor{gray!20}& & &0.064&0.094 &0.028&0.093 \\
%Pedigree &24 &(853,853,24,5) &0.033 &0.028&0.021&0.021\\
%\rowcolor{gray!20}& & &0.292 &0.245&0.234 &0.195\\
%Promedas &64 &(618,618,21,2) &0.030&0.042 &0.021&0.033 \\
%\rowcolor{gray!20}& & &0.139&0.207 &0.096&0.153 \\
%DBN &36 &(719,14205,29,2) &0.016 &0.011&2E-6&2E-6\\
%\rowcolor{gray!20}& & &0.766&0.833 &2E-4&2E-4\\
%ObjDetect &79 &(60,210,6,16) &0.018&0.039 &0.009 &0.004\\
%\rowcolor{gray!20}& & &0.189&0.233 &0.061 &0.021\\
%Grids &8 &(250,728,22,2) &- &- &0.056&- \\
%\rowcolor{gray!20}& & &- &- &0.209&- \\
%CSP &12 &(73,369,12,4) &- &- &0.054&0.069 \\
%\rowcolor{gray!20}& & &- &- &0.093 &0.081\\
%Segment &50 &(229,851,17,2) &5E-6&0.002 &5E-6&5E-6\\
%\rowcolor{gray!20}& & &7E-5&0.036 &7E-5&7E-5\\
%Protein &68 &(59,176,6,77) &0.003&0.003&0.001&0.001\\
%\rowcolor{gray!20}& & &0.049 &0.030&0.015 &0.011\\ \midrule
%\#Inst &493 & &485 &488 &487 &489 \\
%\bottomrule
%\end{tabular}
\end{table}


==> tables/runtime.tex <==
\begin{table}[!htp]\centering
\caption{Comparison of average and maximum runtime required for inference using IBIA20 with variational methods LBP and HAK. Entries are marked
as ‘-’ where all instances could not solved within 20 minutes.}\label{tab: }
\small
\begin{tabular}{lrrrrrrrr}\toprule
&Total &\multicolumn{3}{c}{Average Runtime (s)} &\multicolumn{3}{c}{Maximum Runtime (s)} \\\cmidrule{3-8}
&\#Inst &LBP &HAK &IBIA20 &LBP &HAK &IBIA20 \\\midrule
BN &97 &11 &- &5 &272 &- &43 \\
GridBN &29 &0.02 &13 &2 &0.1 &110 &7 \\
Bnlearn &26 &0.04 &4 &1 &0.2 &22 &2 \\
Pedigree &24 &3 &2 &24 &55 &8 &72 \\
Promedas &64 &0.01 &2 &14 &0.04 &6 &79 \\
DBN &36 &- &1.6 &30 &- &1.9 &44 \\
Object Detection &79 &0.01 &26 &2 &0.02 &70 &4 \\
Grids &8 &3 &0.2 &12 &9 &1 &21 \\
CSP &12 &0.03 &4 &1 &0.2 &15 &4 \\
Segmentation &50 &0.01 &2 &1 &0.02 &5 &5 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/test.tex <==
\begin{table}[!htp]\centering
\caption{Comparison of error in marginals obtained with various inference methods measured using two error metrics. For sampling based methods, we show results with two runtime limits, 2 minutes and 20 minutes. The minimum error obtained for each set in highlighted in bold. Entries are marked as ‘-’ where all instances could not solved within the set time limit.}
\label{tab:avgHD}
\begin{subtable}{\textwidth}
\caption{Average of the mean Hellinger distance over all instances in each set.}\label{tab:avgHD}
\label{tab:}
\scriptsize
\setlength\tabcolsep{3pt}
\begin{tabular}{lrrrrrrr|rrrrrrrr}\toprule
\multirow{2}{*}{} &Total &\multicolumn{6}{c|}{2 minutes} &\multicolumn{6}{c}{20 minutes} & \\\cmidrule{3-15}
&\#Inst &LBP &HAK &ARB &ISSwc20 &ISSwcd &IBIA20 &LBP &HAK &ARB &ISSwc20 &ISSwcd &IBIA20 &IBIA23 \\\midrule
BN &97 &- &- &- &0.037 &- &\textbf{2E-4} &0.023 &- &- &0.033 &- &2E-4 &\textbf{6E-5} \\
GridBN &29 &0.075 &0.018 &0.169 &0.005 &0.003 &\textbf{5E-6} &0.075 &- &0.167 &0.005 &0.001 &5E-6 &\textbf{2E-7} \\
Bnlearn &26 &0.010 &0.021 &- &0.036 &0.012 &\textbf{7E-5} &0.010 &0.010 &- &0.036 &0.006 &7E-5 &\textbf{7E-6} \\
Pedigree &24 &0.075 &0.034 &0.099 &0.028 &0.033 &\textbf{0.009} &0.075 &0.036 &0.086 &0.021 &0.021 &0.009 &\textbf{0.008} \\
Promedas &64 &0.032 &0.033 &0.168 &0.042 &0.030 &\textbf{0.013} &0.032 &0.032 &0.152 &0.033 &0.021 &0.013 &\textbf{0.010} \\
DBN &36 &- &0.284 &0.289 &\textbf{0.011} &0.016 &0.020 &- &0.284 &0.293 &\textbf{2E-6} &\textbf{2E-6} &0.020 &0.003 \\
Object Detection &79 &0.022 &0.085 &- &0.039 &0.018 &\textbf{0.002} &0.022 &- &- &0.004 &0.009 &0.002 &\textbf{4E-4} \\
Grids &8 &0.433 &0.323 &0.295 &- &- &0.088 &0.433 &0.324 &0.302 &- &0.056 &0.088 &\textbf{0.002} \\
CSP &12 &0.019 &0.038 &- &- &- &\textbf{0.002} &0.019 &0.031 &- &0.069 &0.054 &0.002 &\textbf{2E-4} \\
Segmentation &50 &0.035 &0.007 &0.050 &0.002 &\textbf{5E-6} &6E-5 &0.035 &0.005 &0.157 &5E-6 &5E-6 &6E-5 &\textbf{1E-7} \\
Protein &68 &- &- &- &0.003 &0.003 &\textbf{6E-4} &- &\cellcolor[HTML]{A8A8A8} &- &0.001 &0.001 &6E-4 &\textbf{3E-5} \\
\bottomrule
\end{tabular}
\end{subtable}

\begin{subtable}{\textwidth}
\centering
\caption{Average of maximum absolute error over all instances in each set}\label{tab:maxError}
\scriptsize
\setlength\tabcolsep{3pt}
\begin{tabular}{lrrrrrrr|rrrrrrrr}\toprule
&Total &\multicolumn{6}{c|}{2 minutes} &\multicolumn{6}{c}{20 minutes} & \\\cmidrule{3-15}
&\#Inst &LBP &HAK &ARB &ISSwc20 &ISSwcd &IBIA20 &LBP &HAK &ARB &ISSwc20 &ISSwcd &IBIA20 &IBIA23 \\\midrule
BN &97 &- &- &- &0.151 &- &\textbf{0.005} &0.201 &- &- &0.090 &- &0.005 &\textbf{0.001} \\
GridBN &29 &0.474 &0.206 &0.663 &0.073 &0.059 &\textbf{9E-4} &0.474 &- &0.648 &0.053 &0.020 &9E-4 &\textbf{1E-4} \\
Bnlearn &26 &0.068 &0.092 &- &0.093 &0.051 &\textbf{7E-4} &0.068 &0.057 &- &0.092 &0.024 &7E-4 &\textbf{1E-4} \\
Pedigree &24 &0.534 &0.405 &0.631 &0.254 &0.316 &\textbf{0.263} &0.534 &0.401 &0.571 &\textbf{0.211} &0.248 &0.263 &0.242 \\
Promedas &64 &0.166 &0.163 &0.709 &0.220 &0.148 &\textbf{0.080} &0.166 &0.166 &0.654 &0.163 &0.102 &0.080 &\textbf{0.064} \\
DBN &36 &- &0.477 &0.839 &0.833 &0.761 &\textbf{0.287} &- &0.477 &0.813 &\textbf{5E-7} &\textbf{5E-7} &0.287 &0.100 \\
Object Detection &79 &0.081 &0.289 &- &0.195 &0.109 &\textbf{0.009} &0.081 &- &- &0.009 &0.042 &0.009 &\textbf{0.003} \\
Grids &8 &0.940 &0.480 &0.794 &- &- &\textbf{0.339} &0.940 &0.479 &0.837 &- &0.224 &0.339 &\textbf{0.109} \\
CSP &12 &0.061 &0.128 &- &- &- &\textbf{0.006} &0.061 &0.087 &- &0.083 &0.104 &0.006 &\textbf{0.002} \\
Segmentation &50 &0.243 &0.042 &0.686 &0.037 &\textbf{5E-7} &8E-4 &0.243 &0.027 &0.779 &7E-7 &\textbf{5E-7} &8E-4 &\textbf{5E-7} \\
Protein &68 &- &- &- &0.017 &\textbf{0.025} &0.040 &- &\cellcolor[HTML]{A8A8A8} &- &0.005 &0.008 &0.040 &\textbf{8E-4} \\
\bottomrule
\end{tabular}
\end{subtable}
\end{table}

